BiSTNet: Semantic Image Prior Guided Bidirectional Temporal Feature Fusion for Deep Exemplar-based Video Colorization

How to effectively explore the colors of reference exemplars and propagate them to colorize each frame is vital for exemplar-based video colorization. In this paper, we present an effective BiSTNet to explore colors of reference exemplars and utilize them to help video colorization by a bidirectional temporal feature fusion with the guidance of semantic image prior. We first establish the semantic correspondence between each frame and the reference exemplars in deep feature space to explore color information from reference exemplars. Then, to better propagate the colors of reference exemplars into each frame and avoid the inaccurate matches colors from exemplars we develop a simple yet effective bidirectional temporal feature fusion module to better colorize each frame. We note that there usually exist color-bleeding artifacts around the boundaries of the important objects in videos. To overcome this problem, we further develop a mixed expert block to extract semantic information for modeling the object boundaries of frames so that the semantic image prior can better guide the colorization process for better performance. In addition, we develop a multi-scale recurrent block to progressively colorize frames in a coarse-to-fine manner. Extensive experimental results demonstrate that the proposed BiSTNet performs favorably against state-of-the-art methods on the benchmark datasets. Our code will be made available at \url{https://yyang181.github.io/BiSTNet/}

==> Tables/ablation_table1.tex <==


% \begin{table}[bt!]
\begin{table}[]
\begin{center}
\caption{\underline{\textbf{Ablation experiments for the Transformer block}}. PSNR is computed on a high-resolution Urban100 dataset~\cite{huang2015single_urban100}. }
\label{table:ablation main}
\vspace{-2mm}
\setlength{\tabcolsep}{1.3pt}
\scalebox{0.74}{
\begin{tabular}{c | l | c | c | c c c }
\toprule[0.15em]
 &  &  \textbf{FLOPs} &  \textbf{Params} & \multicolumn{3}{c}{\textbf{PSNR}} \\
\cline{5-7}
\textbf{Network} & \hspace{1cm} \textbf{Component} & (B) & (M) & $\sigma$=$15$ & $\sigma$=$25$ & $\sigma$=$50$ \\
\midrule[0.15em]
Baseline & \textbf{\textcolor{blue}{(a)}} UNet with Resblocks~\cite{lim2017enhanced_edsr} & 83.4 & 24.53 & 34.42 &	32.18 &	29.11 \\
\midrule[0.1em]

Multi-head & \textbf{\textcolor{blue}{(b)}} \hspace{0.6cm} MTA + FN~\cite{vaswani2017attention} & 83.7 & 24.84 & 34.66 & 32.39 & 29.28 \\
attention & \textbf{\textcolor{blue}{(c)}} \hspace{0.4cm} MDTA + FN~\cite{vaswani2017attention} & 85.3 & 25.02 & 34.72 & 32.48 & 29.43 \\

\midrule[0.1em]
Feed-forward & \textbf{\textcolor{blue}{(d)}} \hspace{0.55cm} MTA + GFN & 83.5 & 24.79 & 34.70 & 32.43 & 32.40 \\
network & \textbf{\textcolor{blue}{(e)}} \hspace{0.6cm} MTA + DFN & 85.8 & 25.08 & 34.68 & 32.45 & 29.42 \\
 & \textbf{\textcolor{blue}{(f)}} \hspace{0.65cm} MTA + GDFN & 86.2 & 25.12 & 34.77 & 32.56 & 29.54 \\
\midrule[0.1em]
Overall & \textbf{\textcolor{blue}{(g)}} \hspace{0.43cm} MDTA + GDFN & 87.7 & 25.31 & 34.82 & 32.61 & 29.62 \\
\bottomrule[0.1em]
\end{tabular}}
\end{center}
\vspace{-1.5em}
\end{table}




==> Tables/ablation_table2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{table*}[H]
\noindent%
% \begin{table*}[pbt!]
\begin{table*}[bp]
\parbox{.27\textwidth}{
\centering
\captionof{table}{Influence of concat (w/o 1x1 conv) and refinement stage at \underline{\textbf{decoder (level-1)}}. We add the components to experiment Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(g)}}. } 
\label{table:ablation concat}
\vspace{-2mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.7}{
\begin{tabular}{l | c | c | c}
\toprule[0.15em]
 & \textbf{PSNR} ($\sigma$=$50$) & \textbf{FLOPs} & \textbf{Params} \\
\midrule[0.15 em]
Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(g)}} & 29.62 & 87.7 & 25.31 \\
\textbf{+} Concat & 29.66 & 110 & 25.65 \\
\textbf{+} Refinement & 29.71 & 141 & 26.12 \\
\bottomrule[0.1em]
\end{tabular}}
% \scalebox{0.7}{
% \begin{tabular}{l | c  c c}
% \toprule[0.15em]
% Experiment Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(f)}} & \ch & \ch & \ch\\
% Concat  &  & \ch & \ch\\
% Refinement blocks &  & & \ch\\
% \midrule[0.15 em]
% \textbf{PSNR ($\sigma$ = $50$)} & 29.63 & 29.66 & ????? \\
% \bottomrule[0.1em]
% \end{tabular}}
}
\hfill
\parbox{.35\textwidth}{
\centering
\captionof{table}{Results of training \xnet on fixed patch size and progressively large patch sizes. In \underline{\textbf{progressive learning}}~\cite{hoffer2019mix}, we reduce batch size (as patch size increases) to have similar time per optimization step as of fixed patch training. } 
\label{table:ablation progressive}
\vspace{-3mm}
\setlength{\tabcolsep}{2pt}
\scalebox{0.7}{
\begin{tabular}{l | c | c}
\toprule[0.15em]
\textbf{Patch Size} & \textbf{PSNR} ($\sigma$=$50$) & \textbf{Train Time (h)} \\
\midrule[0.15 em]
Fixed ($128^2$) & 29.71 & 22.5\\
Progressive ($128^2$ to $384^2$) & 29.78 & 23.1\\
\bottomrule[0.1em]
\end{tabular}}
}
\hfill
\parbox{.335\textwidth}{
\centering
\captionof{table}{\underline{\textbf{Deeper vs wider}} model. We adjust \# of transformer blocks to keep flops and params constant. Deep narrow model is more accurate, while wide shallow model is faster.} % due to better parallelization.} 
\label{table:ablation deepnarrow}
\vspace{-2mm}
\setlength{\tabcolsep}{4.5pt}
\scalebox{0.7}{
\begin{tabular}{l | c | c | c}
\toprule[0.15em]
\textbf{Dim} & \textbf{PSNR} ($\sigma$=$50$) & \textbf{Train Time (h)} & \textbf{Test Time (s)} \\
\midrule[0.15 em]
48 & \textbf{29.71} & 22.5 & 0.115\\
64 & 29.63 & 15.5 & 0.080\\
80 & 29.56 & \textbf{13.5} & \textbf{0.069}\\
\bottomrule[0.1em]
\end{tabular}}
}
\vspace*{-1em}
\end{table*}

%ps 256x256
% restormer48. 141 flops 0.114979 secs
% restormer64. 143 flops 0.079896 secs
% restormer80. 148 flops 0.068606 secs


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %\begin{table*}[H]
% %
% \begin{minipage}{\textwidth}
% %\begin{table*}[h]
% \parbox{.27\textwidth}{
% \centering
% \captionof{table}{Influence of concat (w/o 1x1 conv) and refinement stage at \underline{\textbf{decoder (level-1)}}. We add the components to experiment Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(g)}}. } 
% \label{table:ablation concat}
% \vspace{-2mm}
% \setlength{\tabcolsep}{2pt}
% \scalebox{0.7}{
% \begin{tabular}{l | c | c | c}
% \toprule[0.15em]
%  & \textbf{PSNR} ($\sigma$=$50$) & \textbf{FLOPs} & \textbf{Params} \\
% \midrule[0.15 em]
% Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(g)}} & 29.62 & 87.7 & 25.31 \\
% \textbf{+} Concat & 29.66 & 110 & 25.65 \\
% \textbf{+} Refinement & 29.71 & 141 & 26.12 \\
% \bottomrule[0.1em]
% \end{tabular}}
% % \scalebox{0.7}{
% % \begin{tabular}{l | c  c c}
% % \toprule[0.15em]
% % Experiment Table~\ref{table:ablation main}\textcolor{blue}{\textbf{(f)}} & \ch & \ch & \ch\\
% % Concat  &  & \ch & \ch\\
% % Refinement blocks &  & & \ch\\
% % \midrule[0.15 em]
% % \textbf{PSNR ($\sigma$ = $50$)} & 29.63 & 29.66 & ????? \\
% % \bottomrule[0.1em]
% % \end{tabular}}
% }
% \hfill
% \parbox{.35\textwidth}{
% \centering
% \captionof{table}{Results of training \xnet on fixed patch size and progressively large patch sizes. In \underline{\textbf{progressive learning}}~\cite{hoffer2019mix}, we reduce batch size (as patch size increases) to have similar time per optimization step as of fixed patch training. } 
% \label{table:ablation progressive}
% \vspace{-3mm}
% \setlength{\tabcolsep}{2pt}
% \scalebox{0.7}{
% \begin{tabular}{l | c | c}
% \toprule[0.15em]
% \textbf{Patch Size} & \textbf{PSNR} ($\sigma$=$50$) & \textbf{Train Time (h)} \\
% \midrule[0.15 em]
% Fixed ($128^2$) & 29.71 & 22.5\\
% Progressive ($128^2$ to $384^2$) & 29.78 & 23.1\\
% \bottomrule[0.1em]
% \end{tabular}}
% }
% \hfill
% \parbox{.335\textwidth}{
% \centering
% \captionof{table}{\underline{\textbf{Deeper vs wider}} model. We adjust \# of transformer blocks to keep flops and params constant. Deep narrow model is more accurate, while wide shallow model is faster.} % due to better parallelization.} 
% \label{table:ablation deepnarrow}
% \vspace{-2mm}
% \setlength{\tabcolsep}{4.5pt}
% \scalebox{0.7}{
% \begin{tabular}{l | c | c | c}
% \toprule[0.15em]
% \textbf{Dim} & \textbf{PSNR} ($\sigma$=$50$) & \textbf{Train Time (h)} & \textbf{Test Time (s)} \\
% \midrule[0.15 em]
% 48 & \textbf{29.71} & 22.5 & 0.115\\
% 64 & 29.63 & 15.5 & 0.080\\
% 80 & 29.56 & \textbf{13.5} & \textbf{0.069}\\
% \bottomrule[0.1em]
% \end{tabular}}
% }
% \vspace*{-1em}
% %\end{table*}
% \end{minipage}


==> Tables/deblurring_table.tex <==

\begin{table}[!t]
\begin{center}
\caption{\small \underline{\textbf{Single-image motion deblurring}} results. Our \xnet is trained only on the GoPro dataset~\cite{gopro2017} and directly applied to the HIDE~\cite{shen2019human} and RealBlur~\cite{rim_2020_realblur} benchmark datasets.}
\label{table:deblurring}
\vspace{-3mm}
\setlength{\tabcolsep}{1.9pt}
\scalebox{0.69}{
\begin{tabular}{l c | c | c | c }
\toprule[0.15em]
 & \textbf{GoPro}~\cite{gopro2017} & \textbf{HIDE}~\cite{shen2019human} & \textbf{RealBlur-R}~\cite{rim_2020_realblur} & \textbf{\textbf{RealBlur-J}}~\cite{rim_2020_realblur} \\
 \textbf{Method} & PSNR~\colorbox{color4}{SSIM} & PSNR~\colorbox{color4}{SSIM} & PSNR~\colorbox{color4}{SSIM} & PSNR~\colorbox{color4}{SSIM}\\
\midrule[0.15em]
Xu \etal \cite{xu2013unnatural}     & 21.00 \colorbox{color4}{0.741} & -  &   34.46 \colorbox{color4}{0.937} &  27.14 \colorbox{color4}{0.830} \\
DeblurGAN \cite{deblurgan}          & 28.70 \colorbox{color4}{0.858} & 24.51 \colorbox{color4}{0.871} & 33.79 \colorbox{color4}{0.903}  &  27.97 \colorbox{color4}{0.834} \\
Nah \etal \cite{gopro2017}          & 29.08 \colorbox{color4}{0.914} & 25.73 \colorbox{color4}{0.874}  &  32.51 \colorbox{color4}{0.841}  &  27.87 \colorbox{color4}{0.827} \\
Zhang \etal \cite{zhang2018dynamic} & 29.19 \colorbox{color4}{0.931} & - &  35.48 \colorbox{color4}{0.947}  &  27.80 \colorbox{color4}{0.847}\\
\small{DeblurGAN-v2 \cite{deblurganv2}}    & 29.55 \colorbox{color4}{0.934} & 26.61 \colorbox{color4}{0.875} & 35.26 \colorbox{color4}{0.944}  &  28.70 \colorbox{color4}{0.866} \\
SRN~\cite{tao2018scale}             & 30.26 \colorbox{color4}{0.934} & 28.36 \colorbox{color4}{0.915} & 35.66 \colorbox{color4}{0.947} &  28.56  \colorbox{color4}{0.867} \\
Shen \etal \cite{shen2019human}     & -                         & 28.89 \colorbox{color4}{0.930} & -        & -  \\
Gao \etal \cite{gao2019dynamic}     & 30.90 \colorbox{color4}{0.935} &  29.11 \colorbox{color4}{0.913}  & -      & - \\
DBGAN \cite{zhang2020dbgan}         & 31.10 \colorbox{color4}{0.942} & 28.94 \colorbox{color4}{0.915}  & 33.78 \colorbox{color4}{0.909}     & 24.93 \colorbox{color4}{0.745} \\
MT-RNN \cite{mtrnn2020}             & 31.15 \colorbox{color4}{0.945} & 29.15 \colorbox{color4}{0.918}   & 35.79 \colorbox{color4}{0.951}     & 28.44 \colorbox{color4}{0.862}\\
DMPHN \cite{dmphn2019}              & 31.20 \colorbox{color4}{0.940}  & 29.09 \colorbox{color4}{0.924} &  35.70 \colorbox{color4}{0.948} & 28.42 \colorbox{color4}{0.860} \\
Suin \etal \cite{Maitreya2020}      & 31.85 \colorbox{color4}{0.948} & 29.98 \colorbox{color4}{0.930} & -       & - \\
SPAIR~\cite{purohit2021spatially_spair} & 32.06 \colorbox{color4}{0.953} & 30.29 \colorbox{color4}{0.931} & - & \underline{28.81} \colorbox{color4}{\underline{0.875}}\\
MIMO-UNet+~\cite{cho2021rethinking_mimo} & 32.45 \colorbox{color4}{0.957} & 29.99 \colorbox{color4}{0.930} & 35.54 \colorbox{color4}{0.947} & 27.63 \colorbox{color4}{0.837}\\
IPT~\cite{chen2021IPT} & \hspace{-2em} 32.52 \colorbox{color4}{-} & - & - & -\\
MPRNet~\cite{Zamir_2021_CVPR_mprnet} & \underline{32.66} \colorbox{color4}{\underline{0.959}} &	\underline{30.96} \colorbox{color4}{\underline{0.939}} & \underline{35.99}   \colorbox{color4}{\underline{0.952}} & 28.70 \colorbox{color4}{0.873} \\
\bottomrule[0.1em]
\textbf{\xnet} & \textbf{32.92} \colorbox{color4}{\textbf{0.961}} & \textbf{31.22} \colorbox{color4}{\textbf{0.942}} & \textbf{36.19} \colorbox{color4}{\textbf{0.957}} & \textbf{28.96} \colorbox{color4}{\textbf{0.879}}\\
\bottomrule[0.1em]
\end{tabular}}
\end{center}\vspace{-2em}
\end{table}








% \begin{table}[t]
% \begin{center}
% \caption{\small \underline{\textbf{Single image deblurring}} results. Our \xnet is trained only on the GoPro dataset~\cite{gopro2017} and directly applied to the HIDE~\cite{shen2019human} and RealBlur~\cite{rim_2020_realblur} benchmark datasets.}
% \label{table:deblurring}
% \vspace{-2mm}
% \setlength{\tabcolsep}{1.9pt}
% \scalebox{0.69}{
% \begin{tabular}{l c | c | c | c }
% \toprule[0.15em]
%  & \textbf{GoPro}~\cite{gopro2017} & \textbf{HIDE}~\cite{shen2019human} & \textbf{RealBlur-R}~\cite{rim_2020_realblur} & \textbf{\textbf{RealBlur-J}}~\cite{rim_2020_realblur} \\
%  \textbf{Method} & PSNR~\colorbox{gray!20}{SSIM} & PSNR~\colorbox{gray!20}{SSIM} & PSNR~\colorbox{gray!20}{SSIM} & PSNR~\colorbox{gray!20}{SSIM}\\
% \midrule[0.15em]
% Xu \etal \cite{xu2013unnatural}     & 21.00 \colorbox{gray!20}{0.741} & -  &   34.46 \colorbox{gray!20}{0.937} &  27.14 \colorbox{gray!20}{0.830} \\
% DeblurGAN \cite{deblurgan}          & 28.70 \colorbox{gray!20}{0.858} & 24.51 \colorbox{gray!20}{0.871} & 33.79 \colorbox{gray!20}{0.903}  &  27.97 \colorbox{gray!20}{0.834} \\
% Nah \etal \cite{gopro2017}          & 29.08 \colorbox{gray!20}{0.914} & 25.73 \colorbox{gray!20}{0.874}  &  32.51 \colorbox{gray!20}{0.841}  &  27.87 \colorbox{gray!20}{0.827} \\
% Zhang \etal \cite{zhang2018dynamic} & 29.19 \colorbox{gray!20}{0.931} & - &  35.48 \colorbox{gray!20}{0.947}  &  27.80 \colorbox{gray!20}{0.847}\\
% \small{DeblurGAN-v2 \cite{deblurganv2}}    & 29.55 \colorbox{gray!20}{0.934} & 26.61 \colorbox{gray!20}{0.875} & 35.26 \colorbox{gray!20}{0.944}  &  28.70 \colorbox{gray!20}{0.866} \\
% SRN~\cite{tao2018scale}             & 30.26 \colorbox{gray!20}{0.934} & 28.36 \colorbox{gray!20}{0.915} & 35.66 \colorbox{gray!20}{0.947} &  28.56  \colorbox{gray!20}{0.867} \\
% Shen \etal \cite{shen2019human}     & -                         & 28.89 \colorbox{gray!20}{0.930} & -        & -  \\
% Gao \etal \cite{gao2019dynamic}     & 30.90 \colorbox{gray!20}{0.935} &  29.11 \colorbox{gray!20}{0.913}  & \colorbox{gray!20}{\qmarks}      & \colorbox{gray!20}{\qmarks}\\
% DBGAN \cite{zhang2020dbgan}         & 31.10 \colorbox{gray!20}{0.942} & 28.94 \colorbox{gray!20}{0.915}  &\colorbox{gray!20}{\qmarks}       & \colorbox{gray!20}{\qmarks} \\
% MT-RNN \cite{mtrnn2020}             & 31.15 \colorbox{gray!20}{0.945} & 29.15 \colorbox{gray!20}{0.918}  & \colorbox{gray!20}{\qmarks}      & \colorbox{gray!20}{\qmarks}\\
% DMPHN \cite{dmphn2019}              & 31.20 \colorbox{gray!20}{0.940}  & 29.09 \colorbox{gray!20}{0.924} &  35.70 \colorbox{gray!20}{0.948} & 28.42 \colorbox{gray!20}{0.860} \\
% Suin \etal \cite{Maitreya2020}      & 31.85 \colorbox{gray!20}{0.948} & 29.98 \colorbox{gray!20}{0.930} & -       & - \\
% MPRNet~\cite{Zamir_2021_CVPR_mprnet} & 32.66 \colorbox{gray!20}{0.959} &	30.96 \colorbox{gray!20}{0.939}	& 35.99  \colorbox{gray!20}{0.952} & 28.70 \colorbox{gray!20}{0.873} \\
% SPAIR~\cite{purohit2021spatially_spair} & 32.06 \colorbox{gray!20}{0.953} & 30.29 \colorbox{gray!20}{0.931} & - & 28.81 \colorbox{gray!20}{0.875}\\
% MIMO-UNet+~\cite{cho2021rethinking_mimo} & 32.45 \colorbox{gray!20}{0.957} & \colorbox{gray!20}{\qmarks} & \colorbox{gray!20}{\qmarks}       & \colorbox{gray!20}{\qmarks}\\
% \bottomrule[0.1em]
% \textbf{\xnet} & \textbf{\qmarks} \colorbox{gray!20}{\qmarks} & \textbf{\qmarks} \colorbox{gray!20}{\qmarks} & \textbf{\qmarks} \colorbox{gray!20}{\qmarks} & \textbf{\qmarks} \colorbox{gray!20}{\qmarks}\\
% \bottomrule[0.1em]
% \end{tabular}}
% \end{center}\vspace{-1.5em}
% \end{table}




% \begin{table}[t]
% \begin{center}
% \caption{\small \underline{\textbf{Single image deblurring}} results. Our \xnet is trained only on the GoPro dataset~\cite{gopro2017} and directly applied to the HIDE~\cite{shen2019human} and RealBlur~\cite{rim_2020_realblur} benchmark datasets.}
% \label{table:deblurring}
% \vspace{-2mm}
% \setlength{\tabcolsep}{1pt}
% \scalebox{0.69}{
% \begin{tabular}{l c | c | c | c }
% \toprule[0.15em]
%  & GoPro~\cite{gopro2017} & HIDE~\cite{shen2019human} & RealBlur-R~\cite{rim_2020_realblur} & RealBlur-J~\cite{rim_2020_realblur} \\
%  Method & PSNR~\colorbox{gray!20}{(SSIM)} & PSNR~\colorbox{gray!20}{(SSIM)} & PSNR~\colorbox{gray!20}{(SSIM)} & PSNR~\colorbox{gray!20}{(SSIM)}\\
% \midrule[0.15em]
% Xu \etal \cite{xu2013unnatural}     & 21.00 \colorbox{gray!20}{(0.741)} & -  &   34.46 \colorbox{gray!20}{(0.937)} &  27.14 \colorbox{gray!20}{(0.830)} \\
% DeblurGAN \cite{deblurgan}          & 28.70 \colorbox{gray!20}{(0.858)} & 24.51 \colorbox{gray!20}{(0.871)} & 33.79 \colorbox{gray!20}{(0.903)}  &  27.97 \colorbox{gray!20}{(0.834)} \\
% Nah \etal \cite{gopro2017}          & 29.08 \colorbox{gray!20}{(0.914)} & 25.73 \colorbox{gray!20}{(0.874)}  &  32.51 \colorbox{gray!20}{(0.841)}  &  27.87 \colorbox{gray!20}{(0.827)} \\
% Zhang \etal \cite{zhang2018dynamic} & 29.19 \colorbox{gray!20}{(0.931)} & - &  35.48 \colorbox{gray!20}{(0.947)}  &  27.80 \colorbox{gray!20}{(0.847)}\\
% \small{DeblurGAN-v2 \cite{deblurganv2}}    & 29.55 \colorbox{gray!20}{(0.934)} & 26.61 \colorbox{gray!20}{(0.875)} & 35.26 \colorbox{gray!20}{(0.944)}  &  28.70 \colorbox{gray!20}{(0.866)} \\
% SRN~\cite{tao2018scale}             & 30.26 \colorbox{gray!20}{(0.934)} & 28.36 \colorbox{gray!20}{(0.915)} & 35.66 \colorbox{gray!20}{(0.947)} &  28.56  \colorbox{gray!20}{(0.867)} \\
% Shen \etal \cite{shen2019human}     & -                         & 28.89 \colorbox{gray!20}{(0.930)} & -        & -  \\
% Gao \etal \cite{gao2019dynamic}     & 30.90 \colorbox{gray!20}{(0.935)} &  29.11 \colorbox{gray!20}{(0.913)}  & -       & - \\
% DBGAN \cite{zhang2020dbgan}         & 31.10 \colorbox{gray!20}{(0.942)} & 28.94 \colorbox{gray!20}{(0.915)}  & -       & - \\
% MT-RNN \cite{mtrnn2020}             & 31.15 \colorbox{gray!20}{(0.945)} & 29.15 \colorbox{gray!20}{(0.918)}  & -       & - \\
% DMPHN \cite{dmphn2019}              & 31.20 \colorbox{gray!20}{(0.940)}  & 29.09 \colorbox{gray!20}{(0.924)} &  35.70 \colorbox{gray!20}{(0.948)} & 28.42 \colorbox{gray!20}{(0.860)} \\
% Suin \etal \cite{Maitreya2020}      & 31.85 \colorbox{gray!20}{(0.948)} & 29.98 \colorbox{gray!20}{(0.930)} & -       & - \\
% MPRNet~\cite{Zamir_2021_CVPR_mprnet} & 32.66 \colorbox{gray!20}{(0.959)} &	30.96 \colorbox{gray!20}{(0.939)}	& 35.99  \colorbox{gray!20}{(0.952)} & 28.70 \colorbox{gray!20}{(0.873)} \\
% SPAIR~\cite{purohit2021spatially_spair} & 32.06 \colorbox{gray!20}{(0.953)} & 30.29 \colorbox{gray!20}{(0.931)} & - & 28.81 \colorbox{gray!20}{(0.875)}\\
% MIMO-UNet+~\cite{cho2021rethinking_mimo} & 32.45 \colorbox{gray!20}{(0.957)} & \colorbox{gray!20}{(??)} & \colorbox{gray!20}{(??)}       & \colorbox{gray!20}{(??)}\\
% \bottomrule[0.1em]
% \textbf{\xnet} & \colorbox{gray!20}{(??)} & \colorbox{gray!20}{(??)} & \colorbox{gray!20}{(??)} & \colorbox{gray!20}{(??)}\\
% \bottomrule[0.1em]
% \end{tabular}}
% \end{center}\vspace{-1.5em}
% \end{table}



==> Tables/deraining_table.tex <==

\begin{table*}
\begin{center}
\caption{\small \underline{\textbf{Image deraining}} results. When averaged across all five datasets, our \xnet advances state-of-the-art by $1.05$~dB.}
\label{table:deraining}
\vspace{-2mm}
\setlength{\tabcolsep}{9.5pt}
\scalebox{0.7}{
\begin{tabular}{l c c c c c c c c c c || c c}
\toprule[0.15em]
  & \multicolumn{2}{c}{\textbf{Test100}~\cite{zhang2019image}}&\multicolumn{2}{c}{\textbf{Rain100H}~\cite{yang2017deep}}&\multicolumn{2}{c}{\textbf{Rain100L}~\cite{yang2017deep}}&\multicolumn{2}{c}{\textbf{Test2800}~\cite{fu2017removing}}&\multicolumn{2}{c||}{\textbf{Test1200}~\cite{zhang2018density}}&\multicolumn{2}{c}{\textbf{Average}}\\
 \textbf{Method} & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$ & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$\\
\midrule[0.15em]
DerainNet~\cite{fu2017clearing} & 22.77  & 0.810  & 14.92  & 0.592  & 27.03  & 0.884  & 24.31  & 0.861  & 23.38  & 0.835  & 22.48 & 0.796    \\
SEMI~\cite{wei2019semi} & 22.35&0.788& 16.56&0.486& 25.03&0.842& 24.43&0.782& 26.05&0.822 & 22.88 & 0.744 \\
DIDMDN~\cite{zhang2018density} & 22.56&0.818& 17.35&0.524& 25.23&0.741& 28.13&0.867& 29.65&0.901& 24.58 & 0.770 \\
UMRL~\cite{yasarla2019uncertainty} & 24.41&0.829& 26.01&0.832& 29.18&0.923& 29.97&0.905& 30.55&0.910& 28.02 & 0.880 \\
RESCAN~\cite{li2018recurrent} & 25.00&0.835& 26.36&0.786& 29.80&0.881& 31.29&0.904& 30.51&0.882& 28.59 & 0.857 \\
PreNet~\cite{ren2019progressive} & 24.81&0.851& 26.77&0.858& 32.44 & 0.950 & 31.75&0.916& 31.36&0.911& 29.42  & 0.897 \\
MSPFN~\cite{mspfn2020}  & 27.50 & 0.876 & 28.66 & 0.860 & 32.40 & 0.933 & 32.82 & 0.930 & 32.39 & 0.916 & 30.75 & 0.903\\
MPRNet~\cite{Zamir_2021_CVPR_mprnet}  & 30.27 & 0.897 & 30.41 & 0.890 & 36.40 & 0.965 & \underline{33.64} & \underline{0.938} & 32.91 & 0.916 & 32.73 & 0.921 \\
SPAIR~\cite{purohit2021spatially_spair} & \underline{30.35} & \underline{0.909} & \underline{30.95} & \underline{0.892} & \underline{36.93} & \underline{0.969} & 33.34 & 0.936 & \underline{33.04} &\underline{0.922} & \underline{32.91} & \underline{0.926} \\
\midrule
% \textbf{\xnet} & \textbf{32.02} & \qmarks & \textbf{31.48} & \qmarks & \textbf{39.04} & \qmarks & \textbf{34.21} & \qmarks & \textbf{33.22} & \qmarks & \textbf{34.00} & \qmarks \\
\textbf{\xnet} & \textbf{32.00} & \textbf{0.923} & \textbf{31.46} & \textbf{0.904} & \textbf{38.99} & \textbf{0.978} & \textbf{34.18} & \textbf{0.944} & \textbf{33.19} & \textbf{0.926} & \textbf{33.96} & \textbf{0.935} \\
\bottomrule[0.1em]
\end{tabular}}
\end{center}\vspace{-1.5em}
\end{table*}


==> Tables/dualpixel_deblurring_table.tex <==


\begin{table*}[!t]
\begin{center}
\caption{\underline{\textbf{Defocus deblurring}} comparisons on the DPDD testset~\cite{abdullah2020dpdd} (containing 37 indoor and 39 outdoor scenes). \textbf{S:} single-image defocus deblurring. \textbf{D:} dual-pixel defocus deblurring. \xnet sets new state-of-the-art for both single-image and dual pixel defocus deblurring. 
}
\label{table:dpdeblurring}
\vspace{-2mm}
\setlength{\tabcolsep}{10pt}
\scalebox{0.7}{
\begin{tabular}{l | c c c c | c c c c | c c c c }
\toprule[0.15em]
%\rowcolor{color3} 
   & \multicolumn{4}{c|}{\textbf{Indoor Scenes}} & \multicolumn{4}{c|}{\textbf{Outdoor Scenes}} & \multicolumn{4}{c}{\textbf{Combined}} \\
\cline{2-13}
%\rowcolor{color3} 
   \textbf{Method} & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$& MAE~$\textcolor{black}{\downarrow}$ & LPIPS~$\textcolor{black}{\downarrow}$  & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$& MAE~$\textcolor{black}{\downarrow}$ & LPIPS~$\textcolor{black}{\downarrow}$  & PSNR~$\textcolor{black}{\uparrow}$ & SSIM~$\textcolor{black}{\uparrow}$& MAE~$\textcolor{black}{\downarrow}$ & LPIPS~$\textcolor{black}{\downarrow}$   \\
\midrule[0.15em]
EBDB$_S$~\cite{karaali2017edge_EBDB} & 25.77 & 0.772 & 0.040 & 0.297 & 21.25 & 0.599 & 0.058 & 0.373 & 23.45 & 0.683 & 0.049 & 0.336 \\
DMENet$_S$~\cite{lee2019deep_dmenet}  & 25.50 & 0.788 & 0.038 & 0.298 & 21.43 & 0.644 & 0.063 & 0.397 & 23.41 & 0.714 & 0.051 & 0.349 \\
JNB$_S$~\cite{shi2015just_jnb} & 26.73 & 0.828 & 0.031 & 0.273 & 21.10 & 0.608 & 0.064 & 0.355 & 23.84 & 0.715 & 0.048 & 0.315 \\
DPDNet$_S$~\cite{abdullah2020dpdd} &26.54 & 0.816 & 0.031 & 0.239 & 22.25 & 0.682 & 0.056 & 0.313 & 24.34 & 0.747 & 0.044 & 0.277\\
% KPAC$_S$~\cite{son2021single_kpac} & \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  &  \qmarks &  \qmarks  &  \qmarks  & 25.24 & 0.845 & ???  & 0.225\\
KPAC$_S$~\cite{son2021single_kpac} & 27.97 & 0.852 & 0.026 & 0.182 & 22.62 & 0.701 & 0.053 & 0.269 & 25.22 & 0.774 & 0.040 & 0.227 \\
IFAN$_S$~\cite{Lee_2021_CVPRifan} & \underline{28.11}  & \underline{0.861}  & \underline{0.026} & \underline{0.179}  & \underline{22.76}  & \underline{0.720} & \underline{0.052}  & \underline{0.254}  & \underline{25.37} & \underline{0.789} & \underline{0.039} & \underline{0.217}\\
\textbf{Restormer}$_S$& \textbf{28.87}  & \textbf{0.882}  & \textbf{0.025} & \textbf{0.145} & \textbf{23.24}  & \textbf{0.743}  & \textbf{0.050} & \textbf{0.209}  & \textbf{25.98}  & \textbf{0.811}  & \textbf{0.038}  & \textbf{0.178}   \\
\midrule[0.1em]
\midrule[0.1em]
DPDNet$_D$~\cite{abdullah2020dpdd} & 27.48 & 0.849 & 0.029 & 0.189 & 22.90 & 0.726 & 0.052 & 0.255 & 25.13 & 0.786 & 0.041 & 0.223 \\
RDPD$_D$~\cite{abdullah2021rdpd} & 28.10 & 0.843 & 0.027 & 0.210 & 22.82 & 0.704 & 0.053 & 0.298 & 25.39 & 0.772 & 0.040 & 0.255 \\

Uformer$_D$~\cite{wang2021uformer} & 28.23 & 0.860 & 0.026 & 0.199 & 23.10 & 0.728 & 0.051 & 0.285 & 25.65 & 0.795 & 0.039 & 0.243 \\

IFAN$_D$~\cite{Lee_2021_CVPRifan} & \underline{28.66} & \underline{0.868} & \underline{0.025} & \underline{0.172} & \underline{23.46} & \underline{0.743} & \underline{0.049} & \underline{0.240} & \underline{25.99} & \underline{0.804} & \underline{0.037} & \underline{0.207} \\


\textbf{Restormer}$_D$& \textbf{29.48}  & \textbf{0.895}  & \textbf{0.023} & \textbf{0.134} & \textbf{23.97}  & \textbf{0.773}  & \textbf{0.047} & \textbf{0.175}  & \textbf{26.66}  & \textbf{0.833}  & \textbf{0.035}  & \textbf{0.155} \\
\bottomrule[0.1em]
\end{tabular}}
\end{center}
\vspace{-1.5em}
\end{table*}

==> Tables/gaussian_denoising_table.tex <==

\begin{table*}[t]
\parbox{.435\linewidth}{
\centering
\caption{\underline{\textbf{Gaussian grayscale image denoising}} comparisons for two categories of methods. Top super row: learning a single model to handle various noise levels. Bottom super row: training a separate model for each noise level.} 
\label{table:graydenoising}
\vspace{-2mm}
\setlength{\tabcolsep}{1.5pt}
\scalebox{0.7}{
\begin{tabular}{l | c c c | c c c | c c c}
\toprule[0.15em]
   & \multicolumn{3}{c|}{\textbf{Set12}~\cite{DnCNN}} & \multicolumn{3}{c|}{\textbf{BSD68}~\cite{martin2001database_bsd}} & \multicolumn{3}{c}{\textbf{Urban100}~\cite{huang2015single_urban100}} \\
 \cline{2-10}
   \textbf{Method} & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ \\
\midrule[0.15em]
% BM3D~\cite{BM3D}  &32.37 & 29.97 & 26.72 & 31.08 & 28.57 & 25.60 & 32.35 & 29.70 & 25.95 \\
% WNNM~\cite{MCWNNM}  &32.70 & 30.28 & 27.05 & 31.37 & 28.83 & 25.87 & 32.97 & 30.39 & 26.83 \\
DnCNN~\cite{DnCNN}  &32.67 & 30.35 & 27.18 & 31.62 & 29.16 & 26.23 & 32.28 & 29.80 & 26.35\\
FFDNet~\cite{FFDNetPlus}  &32.75 & 30.43 & 27.32 & 31.63 & 29.19 & 26.29 & 32.40 & 29.90 & 26.50\\ %top
IRCNN~\cite{zhang2017learning}  &32.76 & 30.37 & 27.12 & 31.63 & 29.15 & 26.19 & 32.46 & 29.80 & 26.22\\ %top
DRUNet~\cite{zhang2021DPIR}  & \underline{33.25} & \underline{30.94} & \underline{27.90} & \underline{31.91} & \underline{29.48} & \underline{26.59} & \underline{33.44} & \underline{31.11} & \underline{27.96}\\ %top
\textbf{\xnet} & \textbf{33.35}	& \textbf{31.04}	& \textbf{28.01} & \textbf{31.95}	& \textbf{29.51}	& \textbf{26.62} & \textbf{33.67}	& \textbf{31.39}	& \textbf{28.33}\\ 
\midrule[0.1em]
\midrule[0.1em]
% DnCNN~\cite{DnCNN}  &32.86 & 30.44 & 27.18 & 31.73 & 29.23 & 26.23 & 32.64 & 29.95 & 26.26\\
FOCNet~\cite{jia2019focnet}  &33.07 & 30.73 & 27.68 & 31.83 & 29.38 & 26.50 & 33.15 & 30.64 & 27.40\\
MWCNN~\cite{liu2018MWCNN}  &33.15 & 30.79 & 27.74 & 31.86 & 29.41 & 26.53 & 33.17 & 30.66 & 27.42\\
% N3Net~\cite{plotz2018N3Net}  &- & 30.55 & 27.43 & - & 29.30 & 26.39 & - & 30.19 & 26.82\\
NLRN~\cite{liu2018NLRN}  &33.16 & 30.80 & 27.64 & 31.88 & 29.41 & 26.47 & 33.45 & 30.94 & 27.49\\
RNAN~\cite{zhang2019residual}  &- & - & 27.70 & - & - & 26.48 & - & - & 27.65\\
DeamNet~\cite{ren2021adaptivedeamnet}  &33.19 & 30.81 & 27.74 & 31.91 & 29.44 & 26.54 & 33.37 & 30.85 & 27.53 \\
DAGL~\cite{mou2021dynamicDAGL}  &33.28 & 30.93 & 27.81 & 31.93 & 29.46 & 26.51 & 33.79 & 31.39 & 27.97 \\
SwinIR~\cite{liang2021swinir} & \underline{33.36} & \underline{31.01} & \underline{27.91} & \textbf{31.97} & \underline{29.50} & \underline{26.58} & \underline{33.70} & \underline{31.30} & \underline{27.98} \\ 
 \textbf{\xnet} & \textbf{33.42} & \textbf{31.08} & \textbf{28.00} & \underline{31.96} & \textbf{29.52}& \textbf{26.62}& \textbf{33.79} & \textbf{31.46}& \textbf{28.29}\\ 
\bottomrule[0.1em]
\end{tabular}}
}
\hfill
% \parbox{.48\linewidth}{
\parbox{.54\linewidth}{
\centering
\caption{\underline{\textbf{Gaussian color image denoising}}. Our \xnet demonstrates favorable performance among both categories of methods. On Urban dataset~\cite{huang2015single_urban100} for noise level $50$, \xnet yields $0.41$ dB gain over CNN-based DRUNet~\cite{zhang2021DPIR}, and $0.2$ dB over Transformer model SwinIR~\cite{liang2021swinir}.}
\label{table:colordenoising}
\vspace{-2mm}
\setlength{\tabcolsep}{1.5pt}
\scalebox{0.7}{
\begin{tabular}{l | c c c | c c c | c c c | c c c}
\toprule[0.15em]
   & \multicolumn{3}{c|}{\textbf{CBSD68}~\cite{martin2001database_bsd}} & \multicolumn{3}{c|}{\textbf{Kodak24}~\cite{kodak}} & \multicolumn{3}{c|}{\textbf{McMaster}~\cite{zhang2011color_mcmaster}} & \multicolumn{3}{c}{\textbf{Urban100}~\cite{huang2015single_urban100}} \\
 \cline{2-13}
   \textbf{Method} & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ & $\sigma$$=$$15$ & $\sigma$$=$$25$ & $\sigma$$=$$50$ \\
\midrule[0.15em]
% CBM3D~\cite{BM3D}  &33.52 & 30.71 & 27.38 & 34.28 & 32.15 & 28.46 & 34.06 & 31.66 & 28.51 & 33.93 & 31.36 & 27.93 \\
IRCNN~\cite{zhang2017learning}   & 33.86 & 31.16 & 27.86 & 34.69 & 32.18 & 28.93 & 34.58 & 32.18 & 28.91 & 33.78 & 31.20 & 27.70\\
FFDNet~\cite{FFDNetPlus}  &33.87 & 31.21 & 27.96 & 34.63 & 32.13 & 28.98 & 34.66 & 32.35 & 29.18 & 33.83 & 31.40 & 28.05 \\
DnCNN~\cite{DnCNN}  &33.90 & 31.24 & 27.95 & 34.60 & 32.14 & 28.95 & 33.45 & 31.52 & 28.62 & 32.98 & 30.81 & 27.59 \\
DSNet~\cite{peng2019dilated}  & 33.91 & 31.28 & 28.05 & 34.63 & 32.16 & 29.05 & 34.67 & 32.40 & 29.28 & - & - & -\\
DRUNet~\cite{zhang2021DPIR}  & \underline{34.30} & \underline{31.69} & \underline{28.51} & \underline{35.31} & \underline{32.89} & \underline{29.86} & \underline{35.40} & \underline{33.14} & \underline{30.08} & \underline{34.81} & \underline{32.60} & \underline{29.61} \\
\textbf{\xnet} & \textbf{34.39} & \textbf{31.78} & \textbf{28.59} & \textbf{35.44} & \textbf{33.02} & \textbf{30.00} & \textbf{35.55} & \textbf{33.31} & \textbf{30.29} & \textbf{35.06} & \textbf{32.91} & \textbf{30.02}\\ 
\midrule[0.1em]
\midrule[0.1em]
RPCNN~\cite{xia2020rpcnn}  &- & 31.24 & 28.06 & - & 32.34 & 29.25 & - & 32.33 & 29.33 & - & 31.81 & 28.62\\
BRDNet~\cite{tian2020BRDnet}  &34.10 & 31.43 & 28.16 & 34.88 & 32.41 & 29.22 & 35.08 & 32.75 & 29.52 & 34.42 & 31.99 & 28.56 \\
RNAN~\cite{zhang2019residual}  &-&-&28.27&-&-&29.58&-&-&29.72&-&-&29.08\\
RDN~\cite{zhang2020rdn}  &-&-&28.31&-&-&29.66&-&-&-&-&-&29.38\\
IPT~\cite{chen2021IPT}  &-&-&28.39&-&-&29.64&-&-&29.98&-&-&29.71\\
SwinIR~\cite{liang2021swinir} & \textbf{34.42} & \underline{31.78} & \underline{28.56} & \underline{35.34} & \underline{32.89} & \underline{29.79} & \underline{35.61} & \underline{33.20} & \underline{30.22} & \underline{35.13} & \underline{32.90} & \underline{29.82} \\
\textbf{\xnet} & \underline{34.40} & \textbf{31.79}& \textbf{28.60}& \textbf{35.47} & \textbf{33.04}& \textbf{30.01}& \textbf{35.61}& \textbf{33.34}& \textbf{30.30} & \textbf{35.13}& \textbf{32.96}& \textbf{30.02}\\ 
\bottomrule[0.1em]
\end{tabular}}
}
\vspace*{-1mm}
\end{table*}


==> Tables/real_denoising_table.tex <==


\begin{table*}[t]
\begin{center}
\caption{\small \small \underline{\textbf{Real image denoising}} on SIDD~\cite{sidd} and DND~\cite{dnd} datasets. \textcolor{red}{$\ast$} denotes methods using additional training data. Our \xnet is trained only on the SIDD images and directly tested on DND. Among competing approaches, only \xnet surpasses $40$~dB PSNR.}
\label{table:realdenoising}
\vspace{-2mm}
\setlength{\tabcolsep}{2.5pt}
\scalebox{0.70}{
\begin{tabular}{c| c| c c c c c c c c c c c c c c c c }
\toprule[0.15em]
& \textbf{ Method} & DnCNN   & BM3D & CBDNet\textcolor{red}{*}   & RIDNet\textcolor{red}{*}  & AINDNet\textcolor{red}{*}  & VDN & SADNet\textcolor{red}{*} &DANet+\textcolor{red}{*} & CycleISP\textcolor{red}{*} & MIRNet & DeamNet\textcolor{red}{*} & MPRNet & DAGL &  Uformer &
 \textbf{\xnet} \\
\textbf{Dataset} & & \cite{DnCNN} & \cite{BM3D} & \cite{CBDNet} & \cite{RIDNet} & \cite{kim2020aindnet} & \cite{VDN} &  \cite{chang2020sadnet}	 & \cite{yue2020danet} &  \cite{zamir2020cycleisp} & \cite{zamir2020mirnet} & \cite{ren2021adaptivedeamnet}& \cite{Zamir_2021_CVPR_mprnet} & \cite{mou2021dynamicDAGL} & \cite{wang2021uformer} & (Ours) \\
\midrule[0.15em]
\textbf{SIDD} & PSNR~$\textcolor{black}{\uparrow}$ &  23.66 &  25.65 & 30.78  &  38.71  &  39.08  & 39.28  & 39.46  & 39.47 & 39.52  & 39.72  & 39.47  & 39.71 & 38.94 & \underline{39.77} & \textbf{40.02} \\
~\cite{sidd}  & SSIM~$\textcolor{black}{\uparrow}$ &  0.583 &  0.685 & 0.801  &  0.951  &  0.954  & 0.956  & 0.957  & 0.957 & 0.957  & 0.959  & 0.957  & 0.958 & 0.953 & \underline{0.959} & \textbf{0.960}\\
\midrule[0.1em]
\textbf{DND} & PSNR~$\textcolor{black}{\uparrow}$ &  32.43 &  34.51 & 38.06  &  39.26  &  39.37  & 39.38  & 39.59  & 39.58 & 39.56  & 39.88  & 39.63  & 39.80 & 39.77 & \underline{39.96} & \textbf{40.03} \\
~\cite{dnd}  & SSIM~$\textcolor{black}{\uparrow}$ &  0.790 &  0.851 & 0.942  &  0.953  &  0.951  & 0.952  & 0.952  & 0.955 & 0.956  & 0.956  & 0.953  & 0.954 & 0.956 & \underline{0.956} & \textbf{0.956} \\
\bottomrule
\end{tabular}}
\end{center}\vspace{-1.5em}
\end{table*}


